SynCron: Efficient Synchronization Support for Near-Data-Processing Architectures

Near-Data-Processing (NDP) architectures present a promising way to alleviate data movement costs and can provide significant performance and energy benefits to parallel applications. Typically, NDP architectures support several NDP units, each including multiple simple cores placed close to memory. To fully leverage the benefits of NDP and achieve high performance for parallel workloads, efficient synchronization among the NDP cores of a system is necessary. However, supporting synchronization in many NDP systems is challenging because they lack shared caches and hardware cache coherence support, which are commonly used for synchronization in multicore systems, and communication across different NDP units can be expensive. This paper comprehensively examines the synchronization problem in NDP systems, and proposes SynCron, an end-to-end synchronization solution for NDP systems. SynCron adds low-cost hardware support near memory for synchronization acceleration, and avoids the need for hardware cache coherence support. SynCron has three components: 1) a specialized cache memory structure to avoid memory accesses for synchronization and minimize latency overheads, 2) a hierarchical message-passing communication protocol to minimize expensive communication across NDP units of the system, and 3) a hardware-only overflow management scheme to avoid performance degradation when hardware resources for synchronization tracking are exceeded. We evaluate SynCron using a variety of parallel workloads, covering various contention scenarios. SynCron improves performance by 1.27$\times$ on average (up to 1.78$\times$) under high-contention scenarios, and by 1.35$\times$ on average (up to 2.29$\times$) under low-contention real applications, compared to state-of-the-art approaches. SynCron reduces system energy consumption by 2.08$\times$ on average (up to 4.25$\times$).

==> discussion.tex <==
\section{\myName{} in Commodity Systems}
\label{Discussionbl}

\revised{In this work, we explore the synchronization problem in NDP systems and we find that they are by nature non-uniform and lack shared caches and hardware cache coherence support. To this end, we design \myName{} to provide hardware synchronization acceleration with a hierarchical communication protocol to tackle non-uniformity of NDP, which is of particular importance in NDP systems for two reasons. First, the strength of NDP systems is the \emph{immense internal bandwidth} inside NDP unit. The external bandwidth across NDP units cannot scale due to the limitation on the number of pins~\cite{Kwon2019TensorDIMM,Kim2013memory}. Thus, as discussed in recent works~\cite{Zhang2018GraphP,Youwei2019GraphQ,Boroumand2019Conda}, excessive traffic across NDP units eventually affects the internal bandwidth utilization, and may significantly delay the NDP execution. Second, NDP configurations based on 3D-stacked memory (only available to several tens of GBs due to technological constraints~\cite{Kwon2019TensorDIMM}) typically include several NDP units~\cite{Kim2013memory,Zhang2018GraphP,Youwei2019GraphQ}, thus incurring high non-uniformity.

The baseline NDP architecture that we assume in this work shares similar key design principles with modern commodity systems which are non-uniform and support explicit message-passing (EMP) instead of cache coherence to share data among cores, e.g., TILE-Gx8036~\cite{petrovic2014leveraging}, SW26010~\cite{Fu2016Sunway}, and the Sunway TaihuLight~\cite{Tang2019plock} system.\cgiannou{More architectures with similar design principles could be added here: (i) Multi-GPUs systems with unified shared memory are also non-coherent and NUMA, (ii) CGRA-based architectures/accelerators are also non-coherent (however they are uniform e.g. Plasticine - ISCA 2017, (iii) disaggregated memory systems (e.g. a multi-threaded workload is partitioned across multiple servers)} However, unlike NDP systems, non-coherent NUMA CPU systems have a shared level of cache, run multiple multi-threaded applications, i.e., a high number software threads executed at hardware threads, and the OS migrates threads between CPU cores to improve system performance. Therefore, although \myName{} could be implemented in them, the proposed hardware design needs to be extended (i) to support the use case scenarios running in these systems, i.e., handling the OS thread migration scenarios among cores and including larger \myTableShort{}s  and waiting lists to satisfy the needs of multiple concurrent multithreaded applications, and  (ii) to exploit the low-cost accesses to caches instead of costly memory accesses to handle overflow scenarios (e.g. leveraging existing technologies like Intel’s CAT~\cite{IntelCAT} \cgiannou{or ARM’s cache lockdown~\cite{ARMCortexA8}} to partition a small portion of the shared cache to be used as a local intermediate cache for overflow scenarios in the \myTableShort{}). We leave the adaptation of \myName{}'s design to other conventional systems that share similar design principles with NDP to future work.}

